Developing the next generation of dual-tip phase-detection probes for air-water flow experiments

Self-aeration is a fascinating phenomenon that commonly occurs in high Froude-number flows in natural or human made environments. The most common air-water flow measurement instrument to characterize such flows is the intrusive dual-tip phase-detection needle probe, which identifies phase changes around the needle tips due to a change of resistivity (phase-detection conductivity probe) or light refraction (phase-detection fiber optical probe). Phase-detection conductivity probes are typically custom made for research purposes, with current design dating back to the 1980ies. In the present study, the next generation of dual-tip conductivity probes is developed and validated against a state-of-the-art system. The novel probe design comprises two main features, including (1) a printed circuit board of the sensor's electrodes and (2) a detachable sensor head. These features offer many advantages over the classical needle-type design. For example, the circuit boards can be manufactured with high precision and the sensor head can be easily replaced in case of damage or deterioration. As such, it is anticipated that this relatively cheap and robust design will enable a better repeatability of air-water flow experiments, combined with an enhanced accessibility for the air-water flow research community.

==> Figures/old/fig1.tex <==
\setlength\extrarowheight{3.7cm}

\begin{longtable}{ p{.47\textwidth}  p{.47\textwidth}} 

\begin{tikzpicture}


\begin{axis}[
        width=9cm,
        height=7cm,
        hide x axis, hide y axis,
        enlargelimits=false,
        axis on top=true,
        ]
      \addplot graphics[xmin=0,ymin=0,xmax=96,ymax=96] {Figures/Q55h20.png};
       \node[rectangle,draw=none,fill=black!30,anchor=north west,text width=\linewidth,minimum height =1cm] (r) at +(0,100) {};
      \node[align=left,anchor=north west,color=white] at (rel axis cs:0,1.0) {\makecell[l]{(\textit{a}) \, 
      \footnotesize{$q = 0.11$ m$^2$/s; $h_\text{gate}/P = 0.5$}}}; 
    \end{axis}
\end{tikzpicture} &

\vspace{-0.5cm}
\end{longtable}




==> Figures/old/tab1n.tex <==
\begin{table}[h]
\begin{footnotesize}
\caption{Key developments of phase-detection intrusive conductivity probes for air-water flow measurements in hydraulic engineering applications; CBR = Canberra}
\begin{tabular}{p{6.5 cm} c p{5 cm} p{6.3 cm} c }
\toprule
Reference &  Institution & Type of air-water flow & Comment \\
\midrule
\citeN{Lamb1950}$^1$, \citeN{Straub1958}$^1$, \citeN{killen1968}$^{1,2}$  & Univ. of Minnesota, US &Smooth laboratory spillway & First development of phase-detection conductivity probes with two different electrodes, separated by 6.35 mm\\
\citeN{Keller1972}$^3$, \citeN{Cain1978}$^4$, \citeN{Cain1981} & Univ. of Canterbury, NZ & Smooth spillway (Aviemore Dam, NZ) & Design adapted from \citeN{Lamb1950}; single-tip probe with $\Phi_\text{in} = 6.35$ m\\
\citeN{Volkart1978}$^5$ &  ETH Zurich, CH & Smooth laboratory spillway & Developed at ETH Zurich \\
\citeN{Tan1984}, \citeN{Low1986} & Univ. of Canterbury, NZ  & Laboratory spillway aerator & Design adapted from previous probes at the Univ. of Canterbury \\
\citeN{Chanson1988}$^6$ & Univ. of Canterbury, NZ & Laboratory spillway aerator & Design adapted from \citeN{Low1986}\\
\citeN{Frizell1994}$^7$, \citeN{Matos1997}$^7$ & Bureau of Reclamation, US  & Laboratory stepped spillway & Design adapted from Univ. of Canterbury probes \\ 
\citeN{Chanson1995}$^8$, \citeN{Cummings1997}$^8$ & Univ. of Queensland, AU & Plunging jet & Design adapted from \citeN{Chanson1988}\\ 
%Boes (2000), Pfister et al. (2006) & ETH Zurich, CH & Laboratory stepped spillway & RBI commercial optical-fiber probe\\
\citeN{Thorwarth2008}$^9$ & RWTH Aachen, GER & Laboratory stepped spillway & Design adapted from \citeN{Chanson1988}\\ 
\citeN{Felder2016}$^{10}$ &   Univ. of New South Wales, AU  &  Laboratory hydraulic jump &  Design adapted from \citeN{Chanson1995}\\
\citeN{Tang2022}$^{11}$ &  Sichuan Univ., CN & Prototype hydraulic jump & Design adapted from \citeN{Chanson1995}\\
Present study$^{12}$ &  Univ. of New South Wales CBR, AU & Submerged hydraulic jump & Developed at UNSW Canberra\\
\bottomrule
\end{tabular}\label{table:intro}
\end{footnotesize}
\footnotesize{
$^2$ Additionally deployed a so-called dipping probe to measure free-surface roughness\\
$^3$ First design of single-tip probe with $\Phi_\text{in} = 6.35$ mm\\
$^4$ Combined probe to measure stagnation pressure and air concentration; 12 mm separation distance between the two electrodes\\
$^5$ Conductivity probe with two different electrodes ($\Phi = 0.5$ mm), separated by 1 mm\\
$^6$ Dual-tip needle conductivity probe with annular needle ($\Phi_\text{out} = 0.8$ mm) and platinum wire ($\Phi_\text{in} = 0.2$ mm) \\
$^7$ Dual-tip needle conductivity probe with stainless steel tube ($\Phi_\text{out} = 1.59$ mm) and platinum wire ($\Phi_\text{in} = 0.2$ mm) \\
$^8$ Dual-tip needle conductivity probe with  annular needle ($\Phi_\text{out} = 0.2$ mm) and platinum wire ($\Phi_\text{in} = 0.025$ mm) \\
$^9$ Dual-tip needle conductivity probe with steel tube ($\Phi_\text{out} = 0.4$ mm) and platinum–iridium electrode ($\Phi_\text{in} = 0.13$ mm)\\
$^{10}$ Dual-tip needle conductivity probe with  annular needle ($\Phi_\text{out} = 0.5$ mm) and platinum wire ($\Phi_\text{in} = 0.125$ mm)\\
$^{11}$ Thick-tip needle conductivity probe with  annular needle ($\Phi_\text{out} = 3$ mm) and xx wire ($\Phi_\text{in} = 1$ mm)\\ 
$^{12}$ NexGen dual-tip phase-detection conductivity probe with gold electrodes; circuit board thickness = 0.2 mm 
}
\end{table}
